Optimal Uniform OPE and Model-based Offline Reinforcement Learning in Time-Homogeneous, Reward-Free and Task-Agnostic Settings

This work studies the statistical limits of uniform convergence for offline policy evaluation (OPE) problems with model-based methods (for episodic MDP) and provides a unified framework towards optimal learning for several well-motivated offline tasks. Uniform OPE $\sup_\Pi|Q^\pi-\hat{Q}^\pi|<\epsilon$ is a stronger measure than the point-wise OPE and ensures offline learning when $\Pi$ contains all policies (the global class). In this paper, we establish an $\Omega(H^2 S/d_m\epsilon^2)$ lower bound (over model-based family) for the global uniform OPE and our main result establishes an upper bound of $\tilde{O}(H^2/d_m\epsilon^2)$ for the \emph{local} uniform convergence that applies to all \emph{near-empirically optimal} policies for the MDPs with \emph{stationary} transition. Here $d_m$ is the minimal marginal state-action probability. Critically, the highlight in achieving the optimal rate $\tilde{O}(H^2/d_m\epsilon^2)$ is our design of \emph{singleton absorbing MDP}, which is a new sharp analysis tool that works with the model-based approach. We generalize such a model-based framework to the new settings: offline task-agnostic and the offline reward-free with optimal complexity $\tilde{O}(H^2\log(K)/d_m\epsilon^2)$ ($K$ is the number of tasks) and $\tilde{O}(H^2S/d_m\epsilon^2)$ respectively. These results provide a unified solution for simultaneously solving different offline RL problems.

==> sections/method.tex <==

% !TEX root = ../Uniform_OPE_icml.tex

\subsection{Tabular Marginalized Importance Sampling Estimator}

\textbf{We stick with the tabular marginalized importance sampling estimator (TMIS). }

In addition to the non-stationary, finite horizon tabular MDP $M=(\mathcal{S},\mathcal{A},r,T,d_1,H)$ (where $S:=|\mathcal{S}|<\infty$ and $A:=|\mathcal{A}|<\infty$), non-stationary logging policy $\mu$ and target policy $\pi$ in Section~\ref{sec:preliminary}, we denote $d^\mu_t(s_t,a_t)$ and $d^\pi_t(s_t,a_t)$ the induced joint state-action distribution at time $t$ and the state distribution counterparts $d^\mu_t(s_t)$ and $d^\pi_t(s_t)$, satisfying $d^{\pi}_t(s_t,a_t)=d^{\pi}_t(s_t)\cdot \pi(a_t|s_t)$.\footnote{For $\mu$, $d^{\mu}_t(s_t,a_t)=d^{\mu}_t(s_t)\cdot \mu(a_t|s_t)$.} The initial distributions are identical $d_1^\mu=d^\pi_1=d_1$. Moreover, we use $P^\pi_{i,j}\in\mathbb{R}^{S\times S}, \;\forall j<i$ to represent the state transition probability from step $j$ to step $i$ under policy $\pi$, where $P^\pi_{t+1,t}(s^\prime|s)=\sum_a P_{t+1,t}(s^\prime|s,a)\pi_t(a|s)$.  The marginal state distribution vector ${d}_t^\pi(\cdot)$ satisfies
${d}_t^\pi  = {P}^{\pi}_{t,t-1} {d}_{t-1}^\pi,$

Historical data $\mathcal{D}=\left\lbrace (s_t^{(i)},a_t^{(i)},r_t^{(i)})\right\rbrace_{i\in[n]}^{t\in[H]} $ was obtained by logging policy $\mu$ and we can only use $\mathcal{D}$ to estimate the value of target policy $\pi$, \emph{i.e.} $v^\pi$. Suppose we only assume knowledge about $\pi(a|s)$ for all $(s,a)\in\mathcal{S}\times\mathcal{A}$ and \emph{do not observe} $r_t(s_t,a_t)$ for any actions other than the noisy immediate reward $r_t^{(i)}$ after observing $s_t^{(i)},a_t^{(i)}$. 

\begin{assumption}[Bounded rewards]\label{assume1}
	 $\forall \;t=1,...,H$ and $i=1,...,n$, $0\leq r^{(i)}_t\leq R_{\max}$.
\end{assumption}
The bounded reward assumption can be relaxed to:  $\exists R_{\max},\sigma<+\infty$ such that $0\leq \mathbb{E}[r_t|s_t,a_t,s_{t+1}]\leq R_{\max}$, $\mathrm{Var}[r_t|s_t,a_t,s_{t+1}]\leq \sigma^2$ (as in \citet{xie2019towards}), for achieving Cramer-Rao lower bound. However, the boundedness will become essential for applying concentrate inequalities in deriving high probability bounds.

\begin{assumption}\label{assume2}
	Logging policy $\mu$ obeys $d_m:=\min_{t,s_t}d^\mu_t(s_t)>0$.
\end{assumption}
This assumption is always required for the consistency of off-policy evaluation estimator. 

\begin{assumption}[Bounded weights]\label{assume3}
	$\tau_s:=\max_{t,s_t}\frac{d^\pi_t(s_t)}{d^\mu_t(s_t)}<+\infty$ and $\tau_a:=\max_{t,s_t,a_t}\frac{\pi(a_t|s_t)}{\mu(a_t|s_t)}<+\infty$.
\end{assumption}
Assumption~\ref{assume3} is also necessary for discrete state and actions, as otherwise the second moments of the importance weight would be unbounded and the MSE of estimators will become intractable . The bound on $\tau_s$ is natural since $\tau_s\leq \max_{t,s_t}\frac{1}{d^\mu_t(s_t)}=\frac{1}{\min_{t,s_t}d^\mu_t(s_t)}=\frac{1}{d_m}$ and it's finite by the Assumption~\ref{assume2}; similarly, $\tau_a<\infty$ is also automatically satisfied if $\min_{t,s_t,a_t}\mu(a_t|s_t)>0$.  

\subsection{Tabular-MIS estimator}

Marginalized importance sampling directly estimates
the marginalized state visitation distribution $\widehat{d}_t$ and defines the MIS estimator:

\begin{equation}\label{MIS_def}
\widehat{v}^\pi_{MIS} =\frac{1}{n}\sum_{i=1}^n\sum_{t=1}^H\frac{\widehat{d}^\pi_t(s_t^{(i)})}{\widehat{d}^\mu_t(s^{(i)}_t)}\widehat{r}^\pi_t(s^{(i)}).
\end{equation}
and $\widehat{d}^\mu_t(\cdot)$ is directly estimated using the empirical mean, \emph{i.e.} $\widehat{d}^\mu_t(s_t):=\frac{1}{n}\sum_i \mathbf{1}(s_t^{(i)}=s_t):=\frac{n_{s_t}}{n}$ whenever $n_{s_t}>0$ and $\widehat{d}^\pi_t(s_t)/\widehat{d}^\mu_t(s_t)=0$ when $n_{s_t}=0$. Then the MIS estimator \eqref{MIS_def} becomes:
\begin{equation}\label{MIS}
\widehat{v}^\pi_{MIS}=\sum_{t=1}^H\sum_{s_t}\widehat{d}^\pi_t(s_t)\widehat{r}^\pi_t(s_t)
\end{equation}

\paragraph{Construction of \TMIS .} 
  
We can construct empirical estimates for $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ as: 
{\small
\begin{equation}\label{eq:tabular_MIS_construction}
%\hspace{-3.5mm}
\begin{aligned}
\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})&=\frac{\sum_{i=1}^n\mathbf{1}[(s^{(i)}_{t+1},a^{(i)}_t,s^{(i)}_t)=(s_{t+1},s_{t},a_{t})]}{n_{s_{t},a_{t}}}\\
\widehat{r}_t(s_t,a_t)&=\frac{\sum_{i=1}^n r_t^{(i)}\mathbf{1}[(s^{(i)}_t,a^{(i)}_t)=(s_t,a_t)]}{n_{s_t,a_t}},\\
\end{aligned}
\end{equation}
}
where we set $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})=0$ and $\widehat{r}_t(s_t,a_t)=0$ if $n_{s_t,a_t}=0$, with $n_{s_t,a_t}$ the empirical visitation frequency to state-action $(s_t,a_t)$ at time $t$. The corresponding estimation of $\widehat{P}_{t+1}(s_{t+1}|s_{t},a_{t})$ and $\widehat{r}_t(s_t,a_t)$ are defined as:

\begin{equation}\label{eq:tabular_MIS_construction2}
\begin{aligned}
\widehat{P}^\pi_t(s_t|&s_{t-1})=\sum_{a_{t-1}}\widehat{P}_t(s_t|s_{t-1},a_{t-1})\pi(a_{t-1}|s_{t-1}),\\
\widehat{r}^\pi_t(s_t)&=\sum_{a_t}\widehat{r}_t(s_t,a_t)\pi(a_t|s_t),\;\widehat{d}^\pi_t=\widehat{P}^\pi_t\widehat{d}^\pi_{t-1}. 
\end{aligned}
\end{equation}




%\red{However, model-based approaches are not well-understood even in tabular setting.  Some discussions and summary of the understanding of tabular methods are here: \url{http://nanjiang.cs.illinois.edu/files/cs598/note3.pdf}
%In particular, check the "Simulation Lemma", and check out the various ``naive approaches'' to analyze the model-based methods.}



==> sections/offline.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex 
%Why do we care about above statistical learning theories? Most critically, Uniform OPE provides theoretical foundation for efficient \emph{offline learning} algorithm.




In this section we discuss the implication of our results on offline learning. As we discussed earlier in the introduction, a uniform OPE bound of $\epsilon$ implies that the corresponding ERM algorithm finds a $2\epsilon$-suboptimal policy.  But it also implies that all other offline policy-learning algorithms that are not ERM, we could gracefully decompose their error into optimization error and statistical  (generalization) error. 
\begin{theorem}\label{thm:offlinelearning}
	Let $\hat{\pi}^* = \argmax_{\pi} \hat{v}^{\pi}$ --- the empirically optimal policy. Let $\hat{\pi}$ be any data-dependent choice of policy such that $\hat{v}^{\hat{\pi}^*} - \hat{v}^{\hat{\pi}} \leq \epsilon_\text{opt}$, then. There is a universal constant $c$ such that w.p. $\geq 1-\delta$ 
	\begin{enumerate}
		\itemsep1pt
		\item 	$
		v^{\pi^*}  - v^{\hat{\pi}} \leq c\sqrt{\frac{H^4S\log(HSA/\delta)}{d_m \cdot n}} + \epsilon_\text{opt}.
		$
		\item If  $\delta< e^{-S}$, the bound improves to $c\sqrt{\frac{H^4S\log(HSA/\delta)}{d_m \cdot n}} +  \epsilon_\text{opt}$. And if in addition $\hat{\pi}$ is deterministic, the bound further improves to 
		$c\sqrt{\frac{H^3\min\{H,S\}\log(HSA/\delta)}{d_m \cdot n}} +  \epsilon_\text{opt}$.
		\item If $\epsilon_\text{opt}\leq \sqrt{H}/S$ and that 
		$||\widehat{V}^{\hat{\pi}}_t-\widehat{V}^{\widehat{\pi}^\star}_t ||_\infty\leq\epsilon_\text{opt},\;\forall t=1,...,H$
		%	$||\widehat{Q}^{\hpi}_1-\widehat{Q}^{\widehat{\pi}^\star}_1 ||_\infty\leq\epsilon_\text{opt} \;\forall t=2,...,H$
		, then 
		$
		v^{\pi^*}  - v^{\hat{\pi}} \leq c\sqrt{\frac{H^3\log(HSA/\delta)}{d_m \cdot n}} + \epsilon_\text{opt}.
		$
	\end{enumerate}
\end{theorem}

\begin{table*}
	\caption{A comparison of related offline policy learning results. }
	\label{table}
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{llll}
			\toprule
			%\multicolumn{2}{c}{Part}                   \\
			\cmidrule(r){1-3}
			Method/Analysis     &Setting& Guarantee     & Sample complexity$^b$ \\
			\midrule
			\cite{agarwal2020model} &Generative model &$\epsilon+O(\epsilon_{\text{opt}}/(1-\gamma))$-optimal  & {$\widetilde{O}(SA/(1-\gamma)^3 \epsilon^2)$}    \\
			\cite{le2019batch,chen2019information} &$\infty$-horizon offline & $\epsilon$-optimal policy  & $\widetilde{O}((1-\gamma)^{-6}C_\mu/ \epsilon^2)$   \\
			\cite{xie2020q} & $\infty$-horizon offline & $\epsilon$-optimal policy  & $\widetilde{O}((1-\gamma)^{-4}C_\mu/ \epsilon^2)$   \\
			{SIMPLEX} for exact empirical optimal$^a$ & $H$-horizon offline  &$\epsilon$-optimal policy & \mypink{$\widetilde{O}(H^3/d_m \epsilon^2)$}    \\
			{PI/VI} for $\epsilon_{\text{opt}}$-empirical optimal  &$H$-horizon offline   & $(\epsilon+\epsilon_{\text{opt}})$-optimal policy & \mypink{$\widetilde{O}(H^3/d_m \epsilon^2)$}    \\
			Minimax lower bound (Theorem~\ref{thm:learn_low_bound})  &$H$-horizon offline    & over class $\mathcal{M}_{d_m}$     & $\Omega(H^3/d_m\epsilon^2)$  \\
			\bottomrule
		\end{tabular}
	}
	\hspace{-4cm}\footnotesize{ $^a$ PI/VI or SIMPLEX is not essential and can be replaced by any efficient empirical MDP solver.}\\
	
	\footnotesize{ $^b$ \emph{Episode} complexity in $H$-horizon setting is comparable to \emph{step} complexity in $\infty$-horizon setting because our finite-horizon MDP is \emph{time-inhomogeneous}.  Informally, we can just take $(1-\gamma)^{-1} \asymp H$ and $C_\mu\asymp 1/d_m$. }
\end{table*}

The third statement implies that all sufficiently accurate planning algorithms based on the empirically estimated MDP are optimal. For example, we can run value iteration or policy iteration to the point that $\epsilon_{\text{opt}} \leq O(H^3/{n d_m})$.  

\noindent\textbf{Comparing to existing work.} Previously no algorithm is known to achieve the optimal sample complexity in the offline setting. Our result also applies to the related generative model setting by replacing $1/d_m$ with $SA$, which avoids the data-splitting procedure usually encountered by specific algorithm design \citep[e.g.,][]{sidford2018near}. 
The analogous policy-learning results In the generative model setting \citep[Theorem 1]{agarwal2020model} , 
 %This analysis has an improvement over \cite{agarwal2020model} as they have a
 achieves a suboptimality of $\tilde{O}(  (1-\gamma)^{-3}SA/n + (1-\gamma)^{-1} \epsilon_{\text{opt}}  )$ with no additional assumption on $ \epsilon_{\text{opt}}$. Informally, if we replace $(1-\gamma)^{-1}$ with $H$, then our result improves the bound from $H \epsilon_{\text{opt}}$ to just $\epsilon_{\text{opt}}$ for $\epsilon_{\text{opt}}\leq \sqrt{H}/S$. 
  %$O(\epsilon_{\text{opt}}/(1-\gamma))$ term which should be translated as $O(\epsilon_{\text{opt}}H)$ in the finite horizon setting. 
  These results are summarized in Table~\ref{table}. 
  
  \noindent\textbf{Sparse MDP estimate.}
  We highlight that the result does not require the estimated MDP to be an accurate approximation in any sense. Recall that the true MDP has $O(S^2)$ parameters (ignoring the dependence on $H,A$ and logarithmic terms), but our result is valid provided that  $n = \tilde{\Omega}(1/d_m)$ which is $\Omega(S)$. This suggests that we may not even exhaustively visit all pairs to state-transitions and that the estimator of $\hat{P}_t$ is allowed to be zero in many coordinates.
  
  
  \noindent\textbf{Optimal computational complexity.}
  Lastly, from the computational perspective, we can leverage the best existing solutions for solving optimization $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$. For example, with $\epsilon_{\text{opt}}>0$, as explained by \citet{agarwal2020model}, value iteration ends in $O(H\log \epsilon_{\text{opt}}^{-1})$ iteration 
  and takes at most $O(HSA)$ time after the model has been estimated with one pass of the data ($O(nH)$ time). We have a total computational complexity of $O(H^4/(d_m \epsilon^2) + H^2SA\log(1/\epsilon))$ time algorithm for obtaining the $\epsilon$-suboptimal policy using $n=O(H^4/(d_m \epsilon^2) $ episodes. This is essentially optimal because the leading term $H^4SA/\epsilon^2$ is required even to just process the data needed for the result to be information-theoretically possible. In comparison, the algorithm that obtains an exact empirical optimal policy $\widehat{\pi}^\star$, the SIMPLEX policy iteration runs in time $O(\text{poly}(H,S,A,n))$ \citep{ye2011simplex}. 
 





% When uniform convergence in OPE is guaranteed, we can derive offline learning algorithms in a straightforward way by learning the empirical optimal policy $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$. As a result, model-based Uniform OPE allows the use of \emph{any} efficient planning algorithm in the empirical MDP, which simplifies algorithm design, as the algorithm utilized need not be tied to the sampling procedure/offline data $\mathcal{D}$. Also, it avoids the data-splitting procedure usually encountered by specific algorithm design, \emph{e.g.} \cite{sidford2018near}. Formally, by leveraging the global Uniform OPE result we have the following:
%
%\begin{theorem}[Offline learning algorithm]\label{thm:offline_learn}
%	Suppose a model-based OPE method $\widehat{v}$ achieves $\epsilon_{\text{uni}}$-uniform convergence, \textit{i.e.} with high probability, $\sup_{\pi\in\Pi} \left|\widehat{v}^\pi-v^\pi\right|\leq \epsilon_{\text{uni}}$. Assuming the realizability that $\pi^\star\in\Pi$. Then by selecting $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$, we obtain with high probability, $
%	v^{\pi^\star}-v^{\widehat{\pi}^\star}\leq 2\epsilon_{\text{uni}}.
%	$ In particular, with OPEMA, if apply Thm~\ref{thm:thre}, then $\widehat{\pi}^\star$ is $\widetilde{O}(\sqrt{H^4S/nd_m})$-optimal policy and if apply Thm~\ref{thm:finer_bound} we know $\widehat{\pi}^\star$ is essentially tighter $\widetilde{O}(\sqrt{H^3S/nd_m})$-optimal policy, regardless of the planning algorithm. 
%\end{theorem}
%The proof was explained in the motivation section before. If $|\Pi|$ is relatively small, we can find $\widehat{\pi}^\star$ with direct policy search: we traverse all the policies $\pi\in\Pi$ and calculate $\widehat{v}^\pi$, and learn the empirical optimal policy $\widehat{\pi}^\star$. If $|\Pi|$ is large, then $\widehat{\pi}^\star:=\text{argmax}_{\pi\in\Pi} \widehat{v}^\pi$ can be solved efficiently by applying standard Policy Iteration (PI) or Value Iteration (VI) on empirical MDP $\widehat{M}$ \citep{sutton2018reinforcement} since $\widehat{M}$ is known. Theorem~\ref{thm:finer_bound} guarantees offline learning with complexity $\widetilde{O}(H^3S/d_m\epsilon^2)$ is one factor away from optimality in learning context (see Theorem~\ref{thm:learn_low_bound} in appendix). 
%
%Theorem~\ref{thm:offline_learn} requires at least one optimal policy to be within the class for the result to work. In contrast, the local uniform convergence result in Theorem~\ref{thm:local_uni_opt} guarantees a $O(\epsilon_{\text{opt}}+\epsilon)$-optimal policy for any policy $\pi$ in the neighborhood of $\widehat{\pi}^\star$ without requirement for optimal policy. Formally, we have the following:
%
%\begin{theorem}\label{thm:uni_opt_local}
%	Suppose $\epsilon_{\text{opt}}\leq \sqrt{H}/S$ and $\widehat{\pi}$ satisfies $||\widehat{Q}^{\hpi}_1-\widehat{Q}^{\widehat{\pi}^\star}_1 ||_\infty\leq\epsilon_\text{opt}$ and $
%	||\widehat{V}^{\hpi}_t-\widehat{V}^{\widehat{\pi}^\star}_t ||_\infty\leq\epsilon_\text{opt},\;\forall t=2,...,H
%	$. There exists constant $c_1,c_2$ such that when $n>c_1H^3\log(HSA/\delta)/d_m\epsilon^2$ with probability $1-\delta$,
%{\small	\[
%	{Q}^{\pi^\star}_1-{Q}_1^{\widehat{\pi}}\leq c_2\cdot \epsilon\cdot\mathbf{1}+\epsilon_{\text{opt}}\cdot\mathbf{1}.
%	\]}
%\end{theorem}
%In the case where $\epsilon_{\text{opt}}=0$, we have $\widehat{\pi}=\widehat{\pi}^\star$ achieves the optimal sample complexity $O(H^3\log(HSA/\delta)/d_m\epsilon^2)$. 







%\twocolumn[text]

==> sections/proof_overview.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex

%\yub{Maybe ``Proof overview'' as the subtitle?}



Our uniform convergence analysis in Section~\ref{sec:mart_con}, relies on creating an unbiased version of $\widehat{v}_\text{OPEMA}$ (which we call it $\widetilde{v}_\text{OPEMA}$) artificially and use concentration (Lemma~\ref{lem:sufficient_sample}) to guarantee $\widehat{v}_\text{OPEMA}$ is identical to $\widetilde{v}_\text{OPEMA}$ in most situations. By doing so we can reduce our analysis from $\sup_{\pi\in\Pi} \left|\widehat{v}^\pi-v^\pi\right|$ to $\sup_{\pi\in\Pi} \left|\widetilde{v}^\pi-v^\pi\right|$. Specifically, $\widetilde{v}^\pi$ replaces  $\widehat{P}_{t}$, $\widehat{r}_t$ in $\widehat{v}^\pi$ by its fictitious counterparts $\widetilde{P}_{t}$, $\widetilde{r}_t$, defined as:
{\small
	\begin{align*}
	\widetilde{r}_t(s_t,a_t)&=\widehat{r}_t(s_t,a_t)\mathbf{1}(E_t)+{r}_t(s_t,a_t)\mathbf{1}(E_t^c),\\
	\widetilde{P}_{t+1}(\cdot|s_t,a_t)&=\widehat{P}_{t+1}(\cdot|s_t,a_t)\mathbf{1}(E_t)+{P}_{t+1}(\cdot|s_t,a_t)\mathbf{1}(E_t^c).
	\end{align*}
}where $E_t$ denotes the event $\{n_{s_t,a_t}\geq nd^\mu_t(s_t,a_t)/2\}$. This is saying, if observation $n_{s_t,a_t}$ is large enough ($E_t$ is true), we use $\widehat{P}$; otherwise we directly use $P$ instead. This track helps dealing with out-of-sample state-action pairs. The next key is the martingale decomposition (Lemma~\ref{lem:martingale_decompose}). On one hand, by using the structure of {\small $\sup_{\pi\in\Pi}\langle{V^\pi_h,(\widetilde{T}_h-T_h)\widetilde{d}^\pi_{h-1}}\rangle$} we can relax it into a ``Rademacher-type complexity'' which corresponds to $\tilde{O}(\sqrt{H^4S/d_m n})$ term in Theorem~\ref{thm:rad}. On the other hand, this decomposition has a natural martingale structure so martingale concentration inequalities can be appropriately applied, \emph{i.e.} Theorem~\ref{thm:single_finer_bound}. In addition, each term {\small $\langle{V^\pi_h,(\widetilde{T}_h-T_h)\widetilde{d}^\pi_{h-1}}\rangle$} separates the non-stationary policy into two parts with empirical distribution only depends on $\pi_{1:h-1}$ that governs how the data ``roll in'' and the long term value function $V^\pi_h$ only depends on $\pi_{h:H}$ that governs how the reward ``roll out''. 

For local uniform convergence, by Bellman equations we can obtain a similar decomposition on $Q$-function:
{
\begin{align*}
\widehat{Q}^\pi_t-Q^\pi_t&=\sum_{h=t+1}^H \Gamma_{t+1:h-1}^\pi(\widehat{P}_{h}-{P}_{h}) \widehat{V}^\pi_{h},
\end{align*}}
where $\Gamma_{t:h}^\pi=\prod_{i=t}^hP^\pi_i$ is the multi-step state-action transition and $\Gamma_{t+1:t}^\pi:=I$. Since $\pi$ is any policy in ${\Pi}_1$ which may dependent on $\mathcal{D}'$ so we cannot directly apply concentration inequalities on $(\widehat{P}_{h}-{P}_{h}) \widehat{V}^\pi_{h}$. Instead, we overcome this hurdle by doing concentration on $(\widehat{P}_{h}-{P}_{h}) \widehat{V}^{\widehat{\pi}^*}_{h}$ since $\widehat{V}^{\widehat{\pi}^*}_{h}$ and $\widehat{P}_{h}$ are independent, and we connect $\widehat{V}^{\widehat{\pi}^*}_{h}$ back to $\widehat{V}^\pi_{h} $ by using they are $\epsilon_\mathrm{opt}$ close (Theorem~\ref{thm:local_uni_opt}). This idea helps avoiding the technicality of absorbing MDP used in \cite{agarwal2020model} for infinite horizon case because of our non-stationary transition setting. For the uniform convergence lower bound, our analysis relies on reducing the problem to identifying $\epsilon$-optimal policy and proving any algorithm that learns a $\epsilon$-optimal policy requires at least $\Omega(H^3/d_m\epsilon^2)$ episodes in the non-stationary episodic setting. Previously, \cite{jiang2017contextual} proves the $\Omega(HSA/\epsilon^2)$ lower bound with assumption $\sum_{i=1}^Hr_i\leq 1$. Our proof uses a modified version of their hard-to-learn MDP instance to achieve the desired result. To produce extra $H^2$ dependence, we leverage the Assumption~\ref{assume1} that $\sum_{i=1}^Hr_i$ may be of order $O(H)$. We only present the high-level ideas here due the space constraint, detailed proofs are explicated in order in Appendix~\ref{sec:the_uni_crude}, \ref{app_sec:mar}, \ref{sec:E}, \ref{sec:lower}.












%\red{Talk about how CR lower bound might not be asymptotically achievable in some cases.}

==> sections/simulation.tex <==
% !TEX root = ../Uniform_convergence_OPE.tex




%\yub{Maybe ``Proof overview'' as the subtitle?}
In this section we use a simple simulated environment to empirically demonstrate the correct scaling in $H$. Direct evaluating $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$ empirically is computationally infeasible since the policy classes we considered here contains either $A^{HS}$ or $\infty$ many policies. 
%For example, if we pick $K$ policies inside the policy class to numerically verify and $K\ll A^{HS}$, then by Lemma~\ref{thm:single_finer_bound} and a union bound, the sup over all $K$ policies is still of order $\widetilde{O}(H^2\log(K))$ (instead of the correct lower bound $\Omega(H^3)$ in Thm~\ref{thm:uni_lower}). 
%To address this issue, 
Instead, in the experiment we will plot the sub-optimality gap $ |v^\star-v^{\widehat{\pi}^\star}|$ with $\hat{\pi}^\star$ being the outputs of policy planning algorithms. The sub-optimality gap is considered as a surrogate for the lower bound of $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$.
%use the learning result and measure $|v^\star-v^{\widehat{\pi}^\star}|$ as a surrogate for $\sup_{\pi\in\Pi} |\widehat{v}^\pi-v^\pi|$. 
Concretely, the non-stationary MDP has $2$ states $s_0,s_1$ and $2$ actions $a_1,a_2$ where action $a_1$ has probability $1$ going back the current state and for action $a_2$, there is one state s.t. after choosing $a_2$ the dynamic transitions to both states with equal probability $\frac{1}{2}$ and the other one has asymmetric probability assignment ($\frac{1}{4}$ and $\frac{3}{4}$). The transition after choosing $a_2$ is changing over different time steps therefore the MDP is non-stationary and the change is decided by a sequence of pseudo-random numbers (Figure~\ref{fig:mdp} shows the transition kernel at a particular time step). Moreover, to make the learning problem non-trivial we use non-stationary rewards with $4$ categories, \emph{i.e.} $r_t(s,a)\in\{\frac{1}{4},\frac{2}{4},\frac{3}{4},1\}$ and assignment of $r_t(s,a)$ for each value is changing over time (see Section~\ref{sec:simluation_detail} in appendix for more details). Lastly, the logging policy in Figure~\ref{fig:different_H} is uniform with $\mu_t(a_1|s)=\mu_t(a_2|s)=\frac{1}{2}$ for both states.


Figure~\ref{fig:different_H} use a fixed number of episodes $n=2048$ while varying $H$ to examine the horizon dependence for uniform OPE. We can see for fixed pointwise OPE with OPEMA (blue line), $|v^\pi-\widehat{v}^\pi|$ scales as $O(\sqrt{H^2})$ which reflects the bound of Lemma~\ref{thm:single_finer_bound}; for the model-based planning, we ran both VI and PI until they converge to the empirical optimal policy $\widehat{\pi}^\star$. %We run both VI/PI for sufficient iterations so they converge to the exact empirical optimal policy $\widehat{\pi}^\star$. 
The figure shows that for this MDP example $|v^\star-v^{\widehat{\pi}^\star}|$ scales as $O(\sqrt{H^3/d_m})$ for fixed $n$ since it is parallel to the reference magenta line. This fact empirically shows $O(\sqrt{H^3/d_m})$ bound is required %for both offline learning and UCOPE and 
confirms the scaling of our theoretical results. 
%For other related simulation %(\emph{e.g.} relative error $|v^\star-v^{\widehat{\pi}^\star}|/v^\star$ for checking experimental correctness), 
%see Appendix~\ref{sec:simluation_detail}.

\begin{figure}
	\centering     %%% not \center
	\subfigure[A non-stationary MDP]{\label{fig:mdp}\includegraphics[width=0.45\linewidth]{MDP-instance.pdf}}
	\subfigure[RMSE vs. Horizon $H$]{\label{fig:different_H}\includegraphics[width=0.5\linewidth]{verify_uniform_convergence.pdf}}
	\caption{Log-log plot  showing the dependence on horizon of uniform OPE and pointwise OPE via learning ($|{v}^{\star}-v^{\widehat{\pi}^\star}|$) over a non-stationary MDP example.}
	\label{fig:main}
\end{figure}


%\red{Talk about how CR lower bound might not be asymptotically achievable in some cases.}
